Unsupervised Domain Adaptation for Keyphrase Generation using Citation Contexts

Adapting keyphrase generation models to new domains typically involves few-shot fine-tuning with in-domain labeled data. However, annotating documents with keyphrases is often prohibitively expensive and impractical, requiring expert annotators. This paper presents silk, an unsupervised method designed to address this issue by extracting silver-standard keyphrases from citation contexts to create synthetic labeled data for domain adaptation. Extensive experiments across three distinct domains demonstrate that our method yields high-quality synthetic samples, resulting in significant and consistent improvements in in-domain performance over strong baselines.

==> figures/bar_chart.tex <==
\begin{tikzpicture}
\pgfplotsset{every tick label/.append style={font=\small}}
\begin{axis}[
    ymin=0,
    ymax=0.4,
    xmin=0,
    xmax=21,
    ybar,
    xtick align=inside,
    xtick={1,5,10,15,20},
    ytick={0.1, 0.2, 0.3, 0.4},
    yticklabels={10\%, 20\%, 30\%, 40\%},
    axis y line*=left,
    bar width=3pt,
    ylabel={\% of documents},
    xlabel={\# of citation contexts},
    ]
\addplot [xshift=-0.5*\pgfplotbarwidth, draw=WildStrawberry!70, fill=WildStrawberry!30] table[col sep=comma, x=nbcc, y=freq]{data/stats.csv};
\end{axis}

\begin{axis}[
    ymin=0,
    ymax=150,
    xmin=0,
    xmax=21,
    ybar,
    xtick align=inside,
    xtick={1,10,20},
    axis y line*=right,
    axis x line*=none,
    bar width=3pt,
    ylabel={\# of candidate phrases},
    ylabel style={rotate=-180}
    ]
\addplot [xshift=0.5*\pgfplotbarwidth, fill=Periwinkle!30, draw=Periwinkle!70] table[col sep=comma, x=nbcc, y=phrases]{data/stats.csv};
\end{axis}



\end{tikzpicture}

==> tables/cross-domains.old.tex <==
\newcolumntype{R}{>{\scriptsize}r}

\begin{tabular}{l| r@{\hspace{.5em}}R@{\hspace{.3em}}R r@{\hspace{.5em}}R@{\hspace{.3em}}R r@{\hspace{.5em}}R@{\hspace{.3em}}R}
\toprule
    \multirow{2}{*}{\textbf{Model}} & 
    \multicolumn{3}{c}{$F_1@M$} & 
    \multicolumn{3}{c}{$F_1@5$} & 
    \multicolumn{3}{c}{$F_1@10$} \\
    \cmidrule(lr){2-4}
    \cmidrule(lr){5-7}
    \cmidrule(lr){8-10}
    ~ &
    all & pres & abs &
    all & pres & abs &
    all & pres & abs \\
\midrule
    BART-FT &
        27.0 & 34.1 & 1.7 &
        26.2 & 31.8 & 2.0 &
        23.4 & 25.8 & 2.5 \\
\cmidrule{1-10}

    +\silk{}~(\texttt{nlp}) & 
    26.7 & 34.8 & 0.8 &
    26.9 & 33.4 & 1.1 &
    24.3 & 27.6 & 1.6 \\
    
    +\silk{}~(\texttt{astro}) & 
    27.6 & 36.0 & 1.0 & 
    27.8 & 34.2 & 1.4 &
    25.0 & 28.1 & 2.0 \\

    +\silk{}~(\texttt{paleo}) &
    26.4 & 34.9 & 0.9 &
    27.1 & 33.5 & 1.4 &
    24.3 & 27.3 & 2.0 \\
\bottomrule
\end{tabular}


% all F@M: 27.0 F@5: 26.2 F@10: 23.4 - bart-kp20k.jsonl
% pre F@M: 34.1 F@5: 31.8 F@10: 25.8 - bart-kp20k.jsonl
% abs F@M:  1.7 F@5:  2.0 F@10:  2.5 - bart-kp20k.jsonl

% all F@M: 26.7 F@5: 26.9 F@10: 24.3 - bart-kp20k.nlp.jsonl
% pre F@M: 34.8 F@5: 33.4 F@10: 27.6 - bart-kp20k.nlp.jsonl
% abs F@M:  0.8 F@5:  1.1 F@10:  1.6 - bart-kp20k.nlp.jsonl

% all F@M: 27.6 F@5: 27.8 F@10: 25.0 - bart-kp20k.astro.jsonl
% pre F@M: 36.0 F@5: 34.2 F@10: 28.1 - bart-kp20k.astro.jsonl
% abs F@M:  1.0 F@5:  1.4 F@10:  2.0 - bart-kp20k.astro.jsonl

% all F@M: 26.4 F@5: 27.1 F@10: 24.3 - bart-kp20k.paleo.jsonl
% pre F@M: 34.9 F@5: 33.5 F@10: 27.3 - bart-kp20k.paleo.jsonl
% abs F@M:  0.9 F@5:  1.4 F@10:  2.0 - bart-kp20k.paleo.jsonl

==> tables/ordering-old.tex <==
\begin{tabular}{l|rrr}
\toprule
     \textbf{Model}  & 
     \textbf{\texttt{nlp}} & 
     \textbf{\texttt{astro}} & 
     \textbf{\texttt{paleo}}  \\
\midrule
    BART-FT    & 26.9 & 16.6 & 18.3 \\
\cmidrule{1-4}
    +\silk{} (top-1K)      & \ssign{30.2} & \ssign{19.5} & 16.8 \\
    +\silk{} (random-1K)   & 29.2 & 18.6 & 17.0 \\
    +\silk{} (bottom-1K)   & 29.0 & \ssign{18.9} & 17.0 \\
\bottomrule
\end{tabular}

% all F@M: 30.8 F@5: 29.8 F@10: 24.8 - bart-base-kp20k-15epochs.jsonl
% all F@M: 31.0 F@5: 29.7 F@10: 25.2 - bart-base-ft-15-nlp-500-3epochs.avg.lr1e-6.jsonl
% all F@M: 27.7 F@5: 25.8 F@10: 20.9 - bart-base-ft-15-nlp.500.bottom.jsonl

% all F@M: 19.1 F@5: 18.6 F@10: 16.5 - bart-base-kp20k-15epochs.jsonl
% all F@M: 18.8 F@5: 19.2 F@10: 17.0 - bart-base-ft-15-astro-500-3epochs.avg.lr1e-6.jsonl
% all F@M: 16.6 F@5: 16.5 F@10: 14.3 - bart-base-ft-15-astro.500.bottom.jsonl

% all F@M: 18.4 F@5: 18.9 F@10: 18.8 - bart-base-kp20k-15epochs.jsonl
% all F@M: 19.0 F@5: 19.3 F@10: 19.2 - bart-base-ft-15-paleo-500-3epochs.avg.lr1e-6.jsonl
% all F@M: 17.7 F@5: 18.6 F@10: 16.5 - bart-base-ft-15-paleo.500.bottom.jsonl

% all F@M: 30.2 F@5: 28.9 F@10: 22.7 - bart-kp20k-ft-aasc-silver-phrases.0.85.0.75.allenai-specter-1000-3epochs.nlp.jsonl
% all F@M: 29.0 F@5: 28.9 F@10: 23.8 - bart-kp20k-ft-nlp.bottom.nlp.jsonl
% all F@M: 28.4 F@5: 29.2 F@10: 24.0 - bart-kp20k-ft-nlp.random.1.nlp.jsonl
% all F@M: 29.4 F@5: 29.5 F@10: 23.7 - bart-kp20k-ft-nlp.random.2.nlp.jsonl
% all F@M: 29.9 F@5: 29.7 F@10: 23.8 - bart-kp20k-ft-nlp.random.3.nlp.jsonl

% all F@M: 19.5 F@5: 20.2 F@10: 17.1 - bart-kp20k-ft-unarxiv-astro-ph-silver-phrases.0.85.0.75.allenai-specter-1000-3epochs.astro.jsonl
% all F@M: 18.9 F@5: 20.2 F@10: 17.3 - bart-kp20k-ft-astro.bottom.astro.jsonl
% all F@M: 18.5 F@5: 19.4 F@10: 16.9 - bart-kp20k-ft-astro.random.1.astro.jsonl
% all F@M: 18.4 F@5: 19.2 F@10: 16.9 - bart-kp20k-ft-astro.random.2.astro.jsonl
% all F@M: 18.9 F@5: 19.5 F@10: 17.0 - bart-kp20k-ft-astro.random.3.astro.jsonl

% all F@M: 17.0 F@5: 18.6 F@10: 18.2 - bart-kp20k-ft-paleo.bottom.paleo.jsonl
% all F@M: 17.2 F@5: 18.7 F@10: 17.6 - bart-kp20k-ft-paleo.random.1.paleo.jsonl
% all F@M: 17.3 F@5: 18.5 F@10: 18.0 - bart-kp20k-ft-paleo.random.2.paleo.jsonl
% all F@M: 16.5 F@5: 18.0 F@10: 17.4 - bart-kp20k-ft-paleo.random.3.paleo.jsonl
% all F@M: 16.8 F@5: 18.7 F@10: 18.1 - bart-kp20k-ft-paleo.s2.0.85.0.60-1000-3epochs.paleo.jsonl




==> tables/venues-for-gold.tex <==
\begin{tabular}{r|lrr}
\toprule
    \textbf{Venue}  & \textbf{Session / Volume} &  \textbf{\#nb} \\
\midrule
    SIGIR 2023 & Language Models & 6 \\
               & Question Answering & 3 \\
               & Summarization \& Text Generation & 5 \\
               & Short Research Papers (manually filtered) & 16 \\
    CIKM 2023  & Natural Language & 24 \\
    WSDM 2023  & Language Models and Text Mining & 6 \\
    SIGIR 2022 & NLP and Semantics & 8 \\
               & Question Answering & 4 \\
               & Sentiment Analysis and Classification & 5 \\
               & Short Research Papers (manually filtered) & 14 \\
    CHI 2022   & Natural Language & 5 \\
    LREC 2022  & Oral sessions (manually filtered) & 81 \\
    NLP Journal\footnote{\url{https://www.sciencedirect.com/journal/natural-language-processing-journal}} & Volumes 2-5 & 35 \\
\bottomrule
    & Total & 212 \\
\bottomrule
\end{tabular}

\begin{tabular}{r|lr}
\toprule
    \textbf{Conference / Journal}  & \textbf{Track / Session} & \textbf{\#nb} \\
\midrule
    arXiv (oct.$\rightarrow$dec. 2023) & astro-ph.HE (High Energy Astrophysical Phenomena)& 20 \\
    ~                                  & astro-ph.CO (Cosmology and Nongalactic Astrophysics) & 20 \\
    ~                                  & astro-ph.IM (Instrumentation and Methods for Astrophysics) & 20 \\
    ~                                  & astro-ph.SR (Solar and Stellar Astrophysics) & 20 \\
    ~                                  & astro-ph.EP (Earth and Planetary Astrophysics) & 20 \\
    ~                                  & astro-ph.GA (Astrophysics of Galaxies) & 20 \\
    Frontiers in Astro. and Space Sc. &  2022-23 Subset selected using arXiv keywords & 76 \\
    %Universe Journal 2022-23 & Solar Systems & 44 \\
    %                        & Planeraty Science & 19 \\
    Astrophysics & 2022-23 & 59 \\
\bottomrule
    & Total & 255 \\
\bottomrule
\end{tabular}

\begin{tabular}{r|lrr}
\toprule
    \textbf{Conference / Journal}  & \textbf{Track / Session} & \textbf{\#nb} \\
\midrule
    Palaeontologia Electronica    & 2023-24 & 21 & OK\\
    Acta Palaeontologica Polonica & 2023 & 22 & ? \\
    Palaeontology                 & 2023 & 26 \\
    Cretaceous Research           & 2024 & 20 \\
    Palaeogeography, Palaeoclimatology, Palaeoecology & 2024 & 47 \\
    Papers in Palaeontology & 2023 & 29 \\
    Proceedings of the Royal Society B: Biological Sciences (paleontology) & 2023 & 25 & OK\\
    Biology Letters (paleontology) & 2023 & 25 & ?\\
    Palaeobiodiversity and Palaeoenvironments & 2023 & 16 & ?\\
\bottomrule
    & Total & 244 \\
\bottomrule
\end{tabular}
